Contextualized Sparse Representations for Real-Time Open-Domain Question Answering

Open-domain question answering can be formulated as a phrase retrieval problem, in which we can expect huge scalability and speed benefit but often suffer from low accuracy due to the limitation of existing phrase representation models. In this paper, we aim to improve the quality of each phrase embedding by augmenting it with a contextualized sparse representation (Sparc). Unlike previous sparse vectors that are term-frequency-based (e.g., tf-idf) or directly learned (only few thousand dimensions), we leverage rectified self-attention to indirectly learn sparse vectors in n-gram vocabulary space. By augmenting the previous phrase retrieval model (Seo et al., 2019) with Sparc, we show 4%+ improvement in CuratedTREC and SQuAD-Open. Our CuratedTREC score is even better than the best known retrieve & read model with at least 45x faster inference speed.

==> _01-intro-old.tex <==
\hanna{edit the text} Currently most NLP models use dense contextualized representations such as BERT, etc. These represenattions are great in many applications, but they do not capture precise lexical information.  Sparse representations (such as tf-idf), on the other hand, have been successfully used in encoding text at sentence or document level, 
capturing precise lexical information that can be sparsely activated by n-gram based features.
%For instance, frequency-based sparse representations such as tf-idf map each text segment to a vocabulary space where the weight of each dimension is determined by the associated word's term and inverse document frequency. 
However, these sparse representations are mainly coarse-grained, task-specific, and  not suitable for word-level representations since they statically assign the identical weight to each n-gram and do not change dynamically depending on the context.

\hanna{edit the following parag}
Many tasks in NLP require both dense and sparse representations. For example, in open-domain question answering, the task of retrieving answer phrases given a web-scale collection of documents, most previous work use a pipeline approach of filtering documents with sparse  tfidf vectors and then use a deep neural model for machine reading comprehension. These methods are great, but slow and they cannot get long tails. 
Most recently, \citet{seo2019real} introduce phrase-indexed real-time question answering that relies on sparse and dense vectors for question answering, but the sparse representations are still document level. The important challenge is how to achieve phrase-level sparse representations at a billion-scale cardinality. 

In this paper, we introduce a method that effectively can learn contextualized phrase-level sparse representations  leveraging rectified self-attention weights on the neighboring  n-grams. Our method  dynamically encodes important lexical information of each phrase (such as named entities) given its context.  
Consequently, in contrast to previous sparse regularization techniques on dense embedding of at most few thousand dimensions~\citep{faruqui2015sparse,subramanian2018spine}, our method is able to produce more interpretable representations to explicitly achieve a sparse representation for each phrase. % each phrasewith billion-scale cardinality. Such large sparse vector space is prohibitive for explicit mapping; 
We leverage the fact that our sparse representations only interact through inner product and \emph{kernelize} the inner-product space for memory-efficient training, inspired by the kernel method in SVMs~\citep{cortes1995support}.
This allows us to handle extremely large sparse vectors without worrying about computational bottlenecks.

We demonstrate the effectiveness of our model in open-domain QA. We adapt the method introduced by 
~\citet{seo2019real} to concatenate both sparse and dense vectors to encode every phrase in Wikipedia and use maximum similarity search to find the closest candidate phrase to answer each question. Our method uses the learned contextualized sparse representation (\ours) instead of the frequency-based features. 
%We only substitute (or augment) the baseline sparse encoding which is entirely based on frequency-based embedding (tf-idf) with our contextualized sparse representation (\ours). 
\hanna{Rewrite the results.}
Our empirical results demonstrate its state-of-the-art performance in open-domain QA datasets, \textsc{SQuAD}$_\textsc{open}$ and \textsc{CuratedTrec}.
Notably, our method significantly outperforms \textsc{DenSPI}~\citep{seo2019real}, the previous end-to-end QA model, by more than 4\% with negligible drop in inference speed. Moreover, our method  achieves up to 2\% better accuracy  and \speedup~speedup in inference compared to pipeline (retrieval-based) approaches. 
Our analysis particularly shows that fine-grained sparse representation is crucial for doing well in phrase retrieval task.



\hanna{two questions: what does dynamically encoding mean? why is your model more interpretable?}

In summary, the contributions of our paper are: (a) we show that learning sparse representations for embedding lexically important context words of a phrase can be achieved by contextualized sparse representations, (b) we introduce an efficient training strategy that leverages the \emph{kernelization} of the sparse inner-product space, and (c) we achieve the state-of-the-art performance in two open-domain QA datasets with up to \speedup~faster inference time.


\hanna{Also think of a teaser figure}

\begin{comment}
Retrieving text from a large collection of documents is an important problem in several natural language tasks such as question answering (QA) and information retrieval. 
% Most recent work in NLP encode phrases using dense vectors that capture syntactic and semantic word-level cues, but do not capture precise lexical information that can be activated with sparse vectors of n-gram based features. 
%
In the literature, sparse representations have been successfully used in encoding text at sentence or document level, 
capturing precise lexical information that can be sparsely activated by n-gram based features.
For instance, frequency-based sparse representations such as tf-idf map each text segment to a vocabulary space where the weight of each dimension is determined by the associated word's term and inverse document frequency.  However, these sparse representations are mainly coarse-grained, task-specific, and  not suitable for word-level representations since they statically assign the identical weight to each n-gram and do not change dynamically depending on the context. %   use similar encoding for every word in the document (or sentence).  These static vectors 



%Other fine-grained hand-engineered features are task-specific and cannot be generalized across different domains. 

%encode every word in the document (or sentence) 
%However, a key limitation of previous methods is that many of them are coarse-grained and defined in document-level. This means that every word in the same document (or sentence) would have exactly the same sparse vector, hence not appropriate for word-level information retrieval tasks. While some other methods have explored more fine-grained features, they are still task-specific and require much human effort that it is not easily generalizable across different domains or tasks.


In this paper, we introduce an effective method for learning a  word-level  sparse representation that encodes precise lexical information. 
Our model, \ours, learns a \emph{co}ntextualized \emph{s}parse \emph{p}hrase \emph{r}epresentation leveraging rectified self-attention weights on the neighboring  n-grams and  dynamically encoding important lexical information of each phrase (such as named entities) given its context. 
Consequently, in contrast to previous sparse regularization techniques on dense embedding of at most few thousand dimensions~\citep{faruqui2015sparse,subramanian2018spine}, our method is able to produce more interpretable representations with billion-scale cardinality. Such large sparse vector space is prohibitive for explicit mapping; we leverage the fact that our sparse representations only interact through inner product and \emph{kernelize} the inner-product space for memory-efficient training, inspired by the kernel method in SVMs~\citep{cortes1995support}.
This allows us to handle extremely large sparse vectors without worrying about computational bottlenecks.
% The overview of our model is illustrated in Figure~\ref{fig:overview}. 

%We adopt \emph{kernel trick} to enable efficient training without explicitly mapping to the extremely large sparse vector space. \hanna{some more interesting insights that you used that help sparse learning} \hanna{is it correct to say that you learn sparse representation using the learned dense vectors? because your self attention is over H, right?}


We demonstrate the effectiveness of our model in open-domain question answering (QA), the task of retrieving answer phrases given a web-scale collection of documents. 
Following~\citet{seo2019real}, we concatenate both sparse and dense vectors to encode every phrase in Wikipedia and use maximum similarity search to find the closest candidate phrase to answer each question.
We only substitute (or augment) the baseline sparse encoding which is entirely based on frequency-based embedding (tf-idf) with our contextualized sparse representation (\ours). 
Our empirical results demonstrate its state-of-the-art performance in open-domain QA datasets, \textsc{SQuAD}$_\textsc{open}$ and \textsc{CuratedTrec}.
Notably, our method significantly outperforms \textsc{DenSPI}~\citep{seo2019real}, the previous end-to-end QA model, by more than 4\% with negligible drop in inference speed. Moreover, our method  achieves up to 2\% better accuracy  and \speedup~speedup in inference compared to pipeline (retrieval-based) approaches. 
Our analysis particularly shows that fine-grained sparse representation is crucial for doing well in phrase retrieval task.
\end{comment}
% Concatenating each dense phrase representation with a paragraph/document-level static sparse representation mitigates the problem to some extent, but we hypothesize that learning finer-grained sparse phrase representations is viable.
% Intuitively, there should be a much smaller number of words that represent the meaning of a phrase, than the number of words in a paragraph or a document.
% Following the distributional hypothesis~\citep{harris1954distributional,firth1957synopsis} which states that ``\textit{a word is characterized by the company it keeps}'', phrases also have such locality.
% Also, the importance of each word in the context of a phrase should change dynamically, but current tf-idf based static sparse representations produce the same sparse representation to all phrases in the same paragraph/document.
%In our experiments, we test our model with kernelized sparse representations on various open-domain question answering benchmarks including $\textsc{SQuAD}_\textsc{open}$, \textsc{CuratedTrec}, and \textsc{NaturalQuestions}.
%We show that our sparse phrase representations largely improve the performance of \textsc{DenSPI} with a negligible amount of increased inference time.
%Combined with our improved training strategy, our proposed model scores over 40\% EM in $\textsc{SQuAD}_\textsc{open}$, which has, compared to BERT-based pipelined models~\citep{yang2019end}, 110x faster inference time with 2.1\% performance gain.

% \begin{figure*}[t!]
% \begin{center}
% \includegraphics[height=5.3cm]{figs/overview_line.pdf}
% \end{center}
% \caption{Overview of our model. Using the billions of precomputed phrase representations, we perform a maximum inner product search between the phrase vectors and an input question vector. We propose to learn contextualized sparse phrase representations which are also very interpretable.}
% \end{figure*}\label{fig:overview}
% \minjoon{Move offline indexing and test time closer to actual vectors}
% \begin{itemize}
%     \item Current trends of pipelined open-domain question answering.
%    \item Emphasizing the problems of pipelined approaches (1. error propagation and 2. speed), describe how phrase reps can be used in open-domain question answering, mitigating pipeline nature of open-domain QA. \hanna{Here, also mention that DensPI is proposed and addresses this problem.}
%    \item Describe the drawback of densely represented phrases \hanna{that is learned by DensPI} as they are difficult to keep exact lexicons in their distributed latent space (entity confusion table here). This is more problematic in open QA due to a large amount of noises.
%    \item Introduce our proposed method, contextualized sparse phrase reps, that dynamically selects lexically important words of a phrase. It uses a kernel trick to avoid using $V$ dimension during training.
%    \item Contributions in three fold: 1) Propose how sparse phrase reps can be trained to embed important lexical info in contexts, 2) show a kernel trick to efficiently train sparse reps, making arbitrary ngram (up to tri in our exp) training possible 3) significantly improves DenSPI in open QA, while keeping latency under 1s.
% \end{itemize}

==> _02-related.tex <==
\paragraph{Open-Domain Question Answering} %While earlier studies in open-domain QA focused on using knowledge base (KB)~\citep{berant2013semantic}, recent development in extractive QA~\citep{rajpurkar2016squad} has opened the possibility of building open-domain QA models with large unstructured texts.\footnote{While there are recent studies on utilizing both KBs and unstructured texts~\citep{sun2018open}, we focus on using only unstructured texts due to its wide applicability to where large-scale KBs are unavailable.}
Most open-domain QA models for unstructured texts use a retriever to find documents to read, and then apply a reading comprehension (RC) model to find answers~\citep{chen2017reading,wang2018r,lin2018denoising,das2018multistep,lee2019latent,yang2019end,wang2019multi}. To improve the performance of the  open-domain question answering, various modifications have been studied to the pipelined models which include improving the retriever-reader interaction~\citep{wang2018r,das2018multistep}, re-ranking paragraphs and/or answers~\citep{wang2018evidence,lin2018denoising,lee2018ranking,kratzwald2019rankqa}, learning end-to-end models with weak supervision~\citep{lee2019latent}, or simply making a better retriever and a reader model~\citep{yang2019end,wang2019multi}.
%They are often combined with additional re-ranking and aggregation models~\citep{wang2018evidence,htut2018training,lee2018ranking,kratzwald2019rankqa} to improve the retrieved documents. 
Due to the pipeline nature, however, these models inevitably suffer error propagation from the retrievers. 

%\hanna{Better comparison with DensPI -- just copied from the old intro}
To mitigate this problem,~\citet{seo2019real} propose to learn  query-agnostic representations of phrases in Wikipedia and retrieve phrases that best answers a question.  While \citet{seo2019real} have shown that encoding both dense and sparse representations for each phrase could keep the lexically important words of a phrase to some extent, their sparse representations are based on static tf-idf vectors which have globally the same weight for each n-gram.
% Although the importance of neighboring n-grams of a phrase should change dynamically depending on its context, tfidf-based static vectors give the same weight to each n-gram in a different context.
% \hanna{Also compare with Kento's emnlp paper}

\paragraph{Phrase Representations} In NLP, phrase representations can be either obtained in a similar manner as word representations~\citep{mikolov2013distributed}, or by learning a parametric function of word representations~\citep{cho2014learning}.
In extractive question answering, phrases are often referred to as spans, but most models do not consider explicitly learning phrase representations as these answer spans can be obtained by predicting only start and end positions in a paragraph~\citep{wang2017machine,seo2017bidirectional}.
Nevertheless, few studies have focused on directly learning and classifying phrase representations~\citep{lee2017learning} which achieve strong performance when combined with attention mechanism.
In this work, we are interested in learning query-agnostic sparse phrase representations which enables the precomputation of re-usable phrase representations~\citep{seo2018phrase}.

\paragraph{Sparse Representations} 
%Due to the discrete nature of text, computational lingustics always has to deal with sparseness of words.
% While the development of distributed dense representations of words have greatly advanced NLP researches~\citep{bengio2003neural,collobert2011natural}, sparse representations of words and phrases have gained relatively fewer attention.
% However, for more coarse-grained texts such as paragraphs or documents, sparse representations are often used to encourage a lexical match between two representations.
One of the most basic sparse representations is the \textit{bag-of-words} modeling, and recent works often emphasize the use of bag-of-words models as strong baselines for sentence classification and question answering~\citep{joulin2017bag,weissenborn2017making}.
\textit{tf-idf} is another good example of sparse representations that is used for document retrieval, and is still widely adopted both in IR and QA community.
Our work could be seen as an attempt to build a trainable tf-idf model for phrase (n-gram) representations, which should be more fine-grained than paragraphs or documents.
There have been some attempts in IR that learn sparse representations of documents for duplicate detection~\citep{hajishirzi2010adaptive}, inverted indexing~\citep{zamani2018neural}, and more.
Unlike previous works, however, our method does not require hand-engineered features for sparse n-grams while keeping the original vocabulary space.
% \hanna{There are some old work in IR community that they try to learn these sparse representations, but they used hand-engineered features (I know of my work at SIGIR'10, but I am sure there are more). The comparison to these IR work is that you are not using any hand-engineered features and hence are generalize. Those methods learn weights of different features by maximing the similarity. } 
In NLP, there are some works on training sparse representations specifically designed for improving interpretability of word representations~\citep{faruqui2015sparse,subramanian2018spine}, but they lose an important role of sparse represenations, which is keeping the exact lexical information, as they are trained by sparsifying dense representations of a higher (but much lower than $V$) dimension.

% \paragraph{Memory-based networks.} It is worth noting that our approach largely resembles the way memory-based networks work.
% The pre-computed billions of phrase vectors are analogous to the memory component in Memory Networks~\citep{weston2015memory,sukhbaatar2015end}.
% In particular, our memory has phrase representations as keys and corresponding phrase strings as values, which could be compared to Key-Value Memory Network (KV-MemNN) by~\citet{miller2016key}, although KV-MemNN depends on KBs for generating memory slots while our model is fully based on unstructured texts.
% \jinhyuk{recent works on LMs as KBs}


% \begin{itemize}
%     \item About pipelined open-domain question answering
%     \item Phrase representations, and its uses in NLP and (open-domain) QA.
%     \item Sparse representations in NLP (mostly used for better interpretability with Lasso), which was not used in QA.
%     \item Memory-based networks as our phrase dumps are related to them.
% \end{itemize}
